Hybrid Adaptive Tuning for Tiered Memory Systems

Memory tiering provides a cost-effective solution to increase memory capacity, utilization, and even bandwidth. Memory tiering relies on system software for memory profiling, detection of frequently accessed pages, and page migration. Such a system software often comes with system parameters. The configurations of those parameters impact application performance. We comprehensively classify system parameters, and characterize the sensitivity of application performance to them using representative memory tiering solutions. Furthermore, we introduce a lightweight and user-friendly framework PTMT, which automates tuning of parameters at runtime for various memory tiering solutions. We identify major challenges for online tuning of memory tiering. PTMT uses a hybrid "offline + online" tuning method: while the offline phase builds a performance database for online queries and reduces runtime overhead, the online phase uses reinforcement learning (customized to memory tiering) to tune. PTMT improves performance by 30%, 26%, 21%, and 14%, on four memory tiering solutions (TPP, UPM, Colloid, and AutoNUMA), compared to using the default configurations. PTMT outperforms the state-of-the-art by 32% on average.

==> figures/tables/LM_performance.tex <==
%\begin{comment}
\begin{table}[]
\small
\caption{Pilot model performance with different model complexity. ``PM'' stands for pilot model. }
\begin{tabular}{c|c|c|c|c}
\hline
\scriptsize{\begin{tabular}[c]{@{}l@{}}PM Complexity\\ (\# of neurons)\end{tabular}} & \scriptsize{\begin{tabular}[c]{@{}l@{}}PM \\Accuracy \end{tabular}}& \scriptsize{\begin{tabular}[c]{@{}l@{}}PM Training\\  Time\end{tabular}} & \scriptsize{\begin{tabular}[c]{@{}l@{}}PM Inference\\ Time\end{tabular}} & \scriptsize{\begin{tabular}[c]{@{}l@{}}PM Memory\\  Consumption \end{tabular}} \\ \hline \hline
256                                                                     &        0.7                &     2h                                                                   &    5us                                                                     &    40KB                                                                        \\ \hline
512                                                                     &  0.82                      &     2.5h                                                                   &     12us                                                                    &    75KB                                                                        \\ \hline
1024                                                                    &        0.88                &       3h                                                                 &     20us                                                                    &      140KB                                                                      \\ \hline
2048                                                                    &       0.91                 &       4h                                                                 &     42us                                                                    &       260KB                                                                     \\ \hline
4096                                                                    &        0.93                &      6h                                                                  &   80us                                                                      &     530KB                                                                       \\ \hline
\end{tabular}
\label{tab:lm_perf}
\end{table}
%\end{comment}

==> figures/tables/feature_selection.tex <==
\begin{table}[h!]
\caption{PCM Metrics and their definitions along with CC values to performance(IPC) \textcolor{sherry}{(make it beautiful and fill up the number)}}\label{tab:feature_selection}
\centering
\begin{tabular}{|c|l|c|}
\hline
\textbf{Metric} & \textbf{Definition} & \textbf{CC} \\ \hline
L3MISS & LLC Misses & 0 \\ \hline
L3MPI & LLC Misses/Instruction & 0 \\ \hline
L3HIT & LLC Hit Rate & 0 \\ \hline
L3OCC & LLC Occupancy & 0 \\ \hline
LMB & Local NUMA Bandwidth & 0 \\ \hline
L2HIT & L2 Cache Hit Rate & 0 \\ \hline
L2MPI & L2 Misses/Instruction & 0 \\ \hline
L2MISS & L2 Misses $\equiv$ CAR & 0 \\ \hline
READ & DRAM read traffic & 0 \\ \hline
WRITE & DRAM write traffic & 0 \\ \hline
PMM\_RD & PMM  read traffic & 0 \\ \hline
PMM\_WR & PMM Memory write traffic & 0 \\ \hline
LLCMISSLAT & LLC Read Miss latency & 0 \\ \hline
RMB & Remote NUMA Bandwidth & 0 \\ \hline
QPI & QPI utilization & 0 \\ \hline
FREQ & CPU frequency & 0 \\ \hline
\end{tabular}

\end{table}
